Leap-Of-Thought: Teaching Pre-Trained Models to Systematically Reason Over Implicit Knowledge

To what extent can a neural network systematically reason over symbolic facts? Evidence suggests that large pre-trained language models (LMs) acquire some reasoning capacity, but this ability is difficult to control. Recently, it has been shown that Transformer-based models succeed in consistent reasoning over explicit symbolic facts, under a "closed-world" assumption. However, in an open-domain setup, it is desirable to tap into the vast reservoir of implicit knowledge already encoded in the parameters of pre-trained LMs. In this work, we provide a first demonstration that LMs can be trained to reliably perform systematic reasoning combining both implicit, pre-trained knowledge and explicit natural language statements. To do this, we describe a procedure for automatically generating datasets that teach a model new reasoning skills, and demonstrate that models learn to effectively perform inference which involves implicit taxonomic and world knowledge, chaining and counting. Finally, we show that "teaching" models to reason generalizes beyond the training distribution: they successfully compose the usage of multiple reasoning skills in single examples. Our work paves a path towards open-domain systems that constantly improve by interacting with users who can instantly correct a model by adding simple natural language statements.

==> 04ab_synthetic-v1.tex <==

We can explore relation between implicit knowledge and reasoning in a more controlled setting by considering rules with synthetic conclusions, such as "is group-1" and "is not group-1". We generate rule sets where, for the entity in question, only one condition is true (core fact) while 3-5 others are false (distractors). E.g.,

\indent{\textbf{Context:} If something often has part wing, then it is a group-1. If something is a material, then it is not a group-1. If something often has part carapace, then it is not a group-1. If something is an insect, then it is a group-1. \textbf{Question:} A toucan is a group-1.}

The rule conclusions have random polarity, with at least one of each. We span three relation types (hypernym, meronym, size comparison), and distractors are sampled to be somewhat adversarial (inverse relation, other relation, etc).

We train a model as before, on a mix of context types (ablating factual statements and rules). The test set is using a distinct hypernym tree of entities from the training set.

Each positive rule condition (e.g, "A toucan often has part wing.") is considered "evidence" for the rule conclusion. We can measure the model's "belief" about the evidence by asking both "in context" of the rules or without any context. As shown in Table~\ref{tab:evidence-correlation}, the accuracy of the evidence is similar in the two cases, only around 10\% of statements do flip between the two, showing that the model makes limited inferences about the facts from the presence of the rules.

\begin{table}[h]
\begin{tabular}{lrrrr}
\toprule
Evidence test & Context free & In context & Amended\\
Evidence accuracy &  81.7 & 86.3 & 94.3\\
\midrule
\textbf{Evidence type} &  &  & \\
All correct & 94.2 (155) & 94.5 (236) & 96.0 (323)\\
No interfering & 97.2 (72) & 96.2 (52) & 93.8 (32)\\
Conflicting & 56.5 (184) & 46.4 (97) & 84.8 (66)\\
Only interfering & 15.4 (13) & 10.3 (39) & 66.7 (3)\\
Any & 75.9 (424) & 75.9 (424) & 93.9 (424)
\bottomrule
\end{tabular}

\caption{Model performance depending on its beliefs about the evidence used in rule conditions. The amended setting adds explicit statements for the 14.5\% incorrect beliefs.
}
\label{tab:evidence-correlation}

\end{table}

In Table~\ref{tab:evidence-correlation} we summarize how the model accuracy depends on its evidence beliefs. We find a very high score when all beliefs are correct, or when an incorrect belief happens to imply the correct rule conclusion. When evidence is inconsistent, the accuracy is near random, and if all evidence points to the wrong conclusion, accuracy is near zero. This shows that to a large extent, the model is internally consistent between implicit knowledge beliefs and applying them to rules.

It is notable that when beliefs are measured in the context of the rules, there are many fewer cases of "conflicting evidence", where multiple rule conditions are met leading to conflicting results. This suggests the model is trying adjust beliefs to create a coherent set.

We can also try to correct the model's incorrect beliefs by supplying them as part of the context. We do this for the 14.5\% incorrect beliefs to create an "amended" test set. The scores increase significantly, although a few of the previously correct beliefs now flip.


==> 04ab_synthetic.tex <==

\subsection{Shortened subsection for the OOV experiments}

In the "real rules" experiments, the model may also have a prior belief about the {\it answer} from pretraining,
adding a potentially confounding element, e.g., is the model right because of reasoning or prior knowledge?.
(We conjecture that this is why the model still occasionally gets the answer right even when all its beliefs
in the rule's conditions are wrong, last line of Table~\ref{??}). To factor this out, we perform another experiment using
rules with out-of-vocabulary (OOV) conclusions of the form {\it "X is in group-N"}. As the
conclusions are OOV, the model has no systematic prior belief in the answers, removing potential answer bias. An example is:
\centerline{
  \begin{tabular}{|ll|} \hline
    \textbf{Context:} & If something often has part wing, then it is a group-1. \\
&    If something is a material, then it is not a group-1. \\
&    If something often has part carapace, then it is not a group-1. \\
&    If something is an insect, then it is a group-1. \\
    \textbf{Question:} &  A toucan is a group-1. \\ \hline
  \end{tabular}
}
\at{I've create a figure example for 4.1 see above, maybe we do the same here?}

We generate rule sets of this form where, for the entity in the question, only one condition is true (core fact) while 3-5 others are false (distractors), and the rule conclusions have random polarity. We then train a model as before. Details are provided in Appendix ?. The test set uses a distinct hypernym tree of entities from the training set. The results are shown in Tables ~?. 
We again observe that correct beliefs almost always lead to correct answers (i.e., imperfect performance can almost always be traced to incorrect beliefs rather than bad reasoning); and that we can largely correct bad answers simply by correcting the incorrect beliefs that led to them, again indicating correct reasoning.

\subsection{original subsection by Oyvind and Pete}
% \pagebreak
\label{subsec:synthetic}
\yg{maybe call these "OOV rules"? or something else that signified ``unknown to model". ``synthetic'' is not very clear imo.}

\jb{I think we should have an appendix with experimental details of this and add those there, and consider making this section a bit shorter}
To remove possible artifacts due to prior knowledge, we perform an additional experiment using rules with synthetic conclusions of the form {\it ``X is in group-N''}. As the conclusions are synthetic, the model cannot reliably answer the question without reasoning with the rules. An example is:

\at{i think we need a data construction, experiments and results in this section as well, for it's different from 4.1. Also should we emphasis that these experiments are about Meronymy?}

\centerline{
  \begin{tabular}{|ll|} \hline
    \textbf{Context:} & If something often has part wing, then it is a group-1. \\
&    If something is a material, then it is not a group-1. \\
&    If something often has part carapace, then it is not a group-1. \\
&    If something is an insect, then it is a group-1. \\
    \textbf{Question:} &  A toucan is a group-1. \\ \hline
  \end{tabular}
}
\at{I've create a figure example for 4.1 see above, maybe we do the same here?}

To correctly answer the question, the model must combine its ``beliefs'' about the rules' conditions (e.g., ``Toucans often have part wing'') - its implicit knowledge - with the explicit rules themselves.

Can a model systematically reason in this way using its implicit beliefs, even if they are wrong? To evaluate this,
we generate rule sets where, for the entity in the question, only one condition is true (core fact) while 3-5 others are false (distractors).
The rule conclusions have random polarity, with at least one of each. We train a model as before, on a mix of context types (ablating factual statements and rules). The test set uses a distinct hypernym tree of entities from the training set.

Once a model is trained, we then probe both the model's implicit beliefs (by a direct query, e.g., ``Toucans often have part wing?''), and its ability to reason with them by posing the rules + question (``A toucan is a group-1?''), for each test case. We find four categories of result:
% Can a model systematically reason in this way using its implicit beliefs, even if they are wrong? To evaluate this, we probed both the model's implicit beliefs (by a direct query, e.g., ``Toucans often have part wing?''), and its ability to reason with them by asking the overall question (``A toucan is a group-1?''). We find four categories of result:
\begin{des}
\item[(a)] the model's relevant beliefs are all correct (hence it should reason to the right answer).
\item[(b)] the model's beliefs are partially correct, but the errors do not lead to a contradictory conclusion (hence it should still get the right answer)
\item[(c)] the model's beliefs are partially correct, and rules both for and against the conclusion are satisfied (here the model behavior is unpredictable)
\item[(d)] the model's beliefs are all/partially incorrect, and {\it consistently} point to the wrong conclusion via the rules (here the model should {\it always} draw the wrong conclusion if reasoning is systematic)
\end{des}
The results are shown in the first two columns of Table~\ref{tab:evidence-correlation}. As an added subtlety, when we probed for the model's beliefs, we found occasionally ($\approx$ 10\% of the cases)  the answer flips depending on whether the question is asked without or with the rules context. \at{this could be in supp} We report results under both conditions (columns 1 and 2). The results show the model {\bf reasons highly systematically} with its implicit beliefs, almost always (94\%+) concluding the right answer when those beliefs consistently point to it (lines 1 and 2), or the opposite answer (83\%+) when those beliefs consistently point against it (line 4), even though those beliefs are wrong.

We also examine whether correcting the (in context) erroneous beliefs, by adding the corrected versions to the rules context, repairs the erroneous conclusions. The results are in column 3 of Table~\ref{tab:evidence-correlation}, indicating that the {\bf corrected beliefs results in corrected reasoning}, and higher overall scores.\footnote{
The few errors arise due to occasional cases of a previously correct belief flipping to incorrect (3\% of the time) when the context was changed; and occasional case of unsystematic reasoning (drawing unwarranted conclusions based on the belief probes). This illustrates that although correctability and systematicity are high, they are not perfect.\at{also to supp probably} } 

% VERSION 1
\eat{
\begin{table}[h]
  \centering
      {
        \begin{tabular}{lrrrr}
  \toprule
{\bf Precision (and \# cases)}  & \multicolumn{2}{|c|}{...with beliefs tested } & ...with corrected \\
{\bf when beliefs are:}  & context free & in context & \multicolumn{1}{c}{beliefs} \\ 
\midrule
\hspace*{3mm} (a)...all correct & 94.2 (155) & 94.5 (236) & 96.0 (323)\\
\hspace*{3mm} (b)...not implying the wrong answer & 97.2 (72) & 96.2 (52) & 93.8 (32)\\
% \hspace*{3mm} (b)...not interfering & 97.2 (72) & 96.2 (52) & 93.8 (32)\\
\hspace*{3mm} (c)...with conflicting implications & 56.5 (184) & 46.4 (97) & 84.8 (66)\\
\hspace*{3mm} (d)...{\it only} implying the wrong answer & 15.4 (13) & 10.3 (39) & 66.7 (3)\\ \hline
% \hspace*{3mm} (d)...only interfering & 15.4 (13) & 10.3 (39) & 66.7 (3)\\ \hline
Overall & 75.9 (424) & 75.9 (424) & 93.9 (424)\\ 
\bottomrule
\end{tabular}
      }
      \vspace{1mm}
\caption{When the model's implicit beliefs consistently imply the right answer via the rules (lines 1 and 2), or the wrong answer (line 4), the model almost always draws that answer, indicating reasoning with implicit knowledge is highly systematic. If we try correcting the incorrect beliefs, \# cases of incorrect answers also drop (column 3).}
\label{tab:evidence-correlation}
\end{table}
}

% VERSION 2 - consolidate Alon's + Oyvind's results
\eat{ 
\begin{table}[h]
  \centering
      {\small
\setlength\tabcolsep{3pt}    	% default 6pt      
        \begin{tabular}{l|rrr|rrr}
\hline
{\bf Precision (and \# cases)} & \multicolumn{3}{|c|}{w/pretrained beliefs} & \multicolumn{3}{|c}{w/corrected beliefs} \\
{\bf when beliefs are:} & Hypernym & Meronym & Mixed & Hypernym & Meronym & Mixed \\
\hline
\hspace*{0mm} (a) ...all correct 						   & 99.9 (1373) & 97.5 (3125) & 99.0 (97) & & & 96.2 (156)\\
\hspace*{0mm} (b)...none imply the wrong answer        & - (0)       & - (0)       & 94.3 (35) & & & - (0)\\
\hspace*{0mm} (c)...with conflicting implications          & 74.1 (434)  & 83.9 (417)  & 44.7 (38) & & & 45.8 (24)\\
\hspace*{0mm} (d)...{\it only} imply wrong answer & 18.8 (32)   & 31.2 (16)   & 16.7 (12) & & & 0.0 (2)\\ \hline
 Overall & & & 81.3 (182) & & & 88.5 (182) \\
\end{tabular}
      }
      \vspace{1mm}
\caption{When the model's implicit beliefs consistently point the right answer via the rules (lines 1 and 2), or the wrong answer (line 4), the model almost always draws that answer, indicating reasoning with implicit knowledge is highly systematic. If we try correcting the incorrect beliefs, \# cases of incorrect answers also drop (column 3).}
\label{tab:evidence-correlation}
\end{table}
} % end eat

% VERSION 2 with PPT Box 
\begin{table}
  \centering
  \includegraphics[width=1\columnwidth]{figures/table.png}
        \vspace{1mm}
\caption{Has the model learned to reason systemetically? If all its implicit beliefs imply right answer, it should answer correctly (green box); and when (incorrect) beliefs consistently imply the {\it wrong} answer, it should answer incorrectly (blue box). We observe this is largely so. If we try correcting the erronous beliefs (columns 4-6), the \# of incorrect answers falls and overall performance improves.}
\label{tab:evidence-correlation}
\end{table}




